Zero-Shot Domain Adaptation in CT Segmentation by Filtered Back Projection Augmentation

Domain shift is one of the most salient challenges in medical computer vision. Due to immense variability in scanners' parameters and imaging protocols, even images obtained from the same person and the same scanner could differ significantly. We address variability in computed tomography (CT) images caused by different convolution kernels used in the reconstruction process, the critical domain shift factor in CT. The choice of a convolution kernel affects pixels' granularity, image smoothness, and noise level. We analyze a dataset of paired CT images, where smooth and sharp images were reconstructed from the same sinograms with different kernels, thus providing identical anatomy but different style. Though identical predictions are desired, we show that the consistency, measured as the average Dice between predictions on pairs, is just 0.54. We propose Filtered Back-Projection Augmentation (FBPAug), a simple and surprisingly efficient approach to augment CT images in sinogram space emulating reconstruction with different kernels. We apply the proposed method in a zero-shot domain adaptation setup and show that the consistency boosts from 0.54 to 0.92 outperforming other augmentation approaches. Neither specific preparation of source domain data nor target domain data is required, so our publicly released FBPAug can be used as a plug-and-play module for zero-shot domain adaptation in any CT-based task.

==> chapters/old.tex <==
ABSTRACT


    % Domain shift is one of the most salient challenges in medical computer vision. Due to immense variability in scanners' parameters and imaging protocols, even images obtained from the same person and the same scanner could differ significantly. We address variability in CT images caused by different convolution kernels used in the reconstruction process, the key domain shift factor in CT. 
    % The choice of a convolution kernel affects pixels' granularity, image smoothness, and noise level. \reconsider{First, we show that U-Net trained on smooth images suffers from the shift to sharp images even for a simple lung segmentation problem.  We analyze paired images, where smooth and sharp images were reconstructed from the same sinograms with different kernels, thus providing identical anatomy but different style. Though identical predictions are desired, we show that the consistency, measured as the average Surface Dice with 1-mm tolerance between predictions on pairs, is just $0.79$. 
    % Second, we propose Filtered Back-Projection Augmentation (FPBAug), a simple and surprisingly efficient physics-driven approach to augment CT images in sinogram space emulating reconstruction with different kernels. 
    % We apply the proposed method in a zero-shot domain adaptation setup and show that the consistency boosts from $0.79$ to $0.93$ preserving quality on the source domain and outperforming other augmentation approaches. Neither specific preparation of source domain data nor target domain data is required, so our publicly released\footnote{\url{https://github.com/STNLd2/FBPAug}} FBPAug can be used as a plug-and-play module for zero-shot domain adaptation in any CT-based problem.}

INTRO



% \begin{figure}[t!]
% \centering
% \includegraphics[width=10cm]{images/pipeline.png}
% \caption{\todo{[doens't linked with the text]} Overview of the proposed Filtered Back Projection Augmentation.}
% \label{fig:sinogr}
% \end{figure}


% \begin{figure}[h]
% \centering
% \includegraphics[width=10cm]{images/4full_slices_red_dots.png}
% \caption{Top left - original image smooth kernel; top right - original image sharp kernel; bot left - image with smooth kernel processed by FBPAug with parameters $a=30,~b=3$; bot right - image with sharp kernel processed by FBPA with parameters $a=-1,~b=0.7$. Red dots represent pixels with $\text{HU} < -950$.}
% \label{fig:slices-red}
% \end{figure}


%\begin{figure}[h]
%\centering
%\includegraphics[width=10cm]{images/hists.png}
%\caption{Intensity distribution of images obtained with smooth (left) and sharp (right) kernels. Blue - original image, orange - sharp to smooth (left) and smooth to sharp (right).}
%\label{fig:hist}
%\end{figure}


% \begin{figure}[h]
% \centering
% \includegraphics[width=10cm]{images/sinogram_to_images.png}
% \caption{Two images obtained from the same sinogram with two different convolution kernels.}
% \label{fig:sinogr}
% \end{figure}


%\begin{enumerate}
%    \item Domain Adaptation...(Not sure, bc this force us to compare with DA methods)
%    \item Short description of CT reconstruction process (?), with emphasis on Conv. Kernels and their impact on a resulting picture.
%    \item List of papers on CT specific augmentations / sinogram keyword (google doc)
%    \item 
%\end{enumerate}


METHOD


% \textbf{NSCLC-Radiomics} dataset \cite{nsclc1} represents a subset of The Cancer Imaging Archive NSCLC Radiomics collection \cite{tcia}. It contains left and right lungs segmentation annotated on 3D thoracic CT series for 402 non-small cell lung cancer (NSCLC) patients. We exclude 79 of them from the analysis since their convolution kernel is unknown (the corresponding DICOM attribute is missing). All the remaining images were acquired with relatively smooth convolution kernels: B18f, B19f, B30f, B31f, B31s, B41f (manufacturer's names) from Siemens scanners.

% \textbf{Moscow Radiology CTLungCa-500} (Cancer-500) dataset \cite{lung-cancer-500} consists of chest CT studies of healthy subjects and patients with lung cancer and some other incidental pathologies (536 studies in total). In contrast with many other public datasets, the majority of studies contain two series (3D CT images); the overall number of series is 980. Most importantly, every pair of series were obtained from one physical scanning with different reconstruction algorithms. It means the slices within these images are perfectly aligned, and the only difference is \textit{style} of the image caused by different convolutional kernels applied. For our experiments, we select 220 patients with 440 paired images (images reconstructed from the raw data, using different convolution kernels) acquired from Toshiba scanners. Soft kernels include FC51, FC55, FC52; sharp kernels - FC07, FC08, FC18 (manufacturer's names). Though the dataset includes lung nodules markers, we ignore this information as all paired series come from healthy patients. 



% \begin{table}[htbp]
% \caption{Datasets summary information.}
% \begin{center}
% \begin{tabular}{l m{30mm} c c}
% \hline
% Dataset & Convolution kernel & Manufacturer \ \ \  & Number of series \\
% %\hline
% %LIDC (sharp) & LUNG & GE & $70$ \\
% %LIDC (soft) & STANDARD & GE & $380$ \\
% \hline
% NSCLC-Rad. (soft)\ \ \  & B18f, B19f, B30f,\newline B31f, B31s, B41f & Siemens & $343$ \\
% \hline
% Cancer-500 (sharp) & FC51, FC55, FC52 & Toshiba & $220$ \\
% Cancer-500 (soft) & FC07, FC08, FC18  & Toshiba & $220$ \\
% \hline
% \end{tabular}
% \end{center}
% \label{tab1:dataset}
% \end{table}

EXPERIMENTS

%\begin{enumerate}
%    \item Lungs (NSCLS->cancer500), nodules (cancer500->cancer500)
%%    \item table with data stats, kernels, number of images, etc
 %   \item Network architecture
 %   \item Training regime
%\end{enumerate}


% \copypaste{In addition to the classical usage as a way to estimate segmentation quality (i.e., to calculate the scores between predictions and ground truth annotation), we also use the same metric to measure the consistency of predictions on the paired kernels (i.e., to calculate the scores between two predictions on the image, reconstructed with two different kernels).}


% multiple images from the same patient, and all images were obtained with relatively soft kernels.  + gt + stat test

%\todo{mibel consider adding as a limitation to conclusion}
%\vskip -20pt
%To answer the first question we train separate networks on LIDC and NSCLC-Radiomics datasets and test their per. 
%For the first experiment we train a cancer segmentation algorithm on a LIDC dataset. We split the dataset into two parts based on convolution kernels "softness". We train neural network on images with "soft" kernels and test them on "hard" and vice versa. For the second experiment, we train lungs' segmentation algorithm on NSCLC Radiomics dataset and make predictions on Cancer-500 dataset paired images. Since there is no lungs' masks provided for Cancer-500, we simply compute agreements between masks for two images from the same pair. Finally, for the last experiment we train a cancer segmentation algorithm  on a LIDC dataset. In all experiments we use 3-fold cross validation to access models performance. To estimate mean and standard deviation of segmentation quality and agreement we use three-fold cross validation.


% \begin{figure}[t!]
% \centering
% \includegraphics[width=10cm]{images/scatter.png}
% \caption{Comparison of agreement scores of FBPAug method and its closest competitor (Noise).}
% \label{fig:agreement}
% \end{figure}

%In the first set of experiments, we use 3-fold cross-validation on \textit{Mosmed-1110}. This dataset is stored in Nifti format and does not contain information about the kernels. Thus, we use it to estimate the in-domain accuracy for COVID-19 segmentation problem.

%\reconsider{
%In the second experiment, we trained the network on the whole Mosmed-1110 and make predictions for the paired images from the Covid-private dataset. Next, we compare masks within each pair of sharp and soft images using Dice score. These metrics estimate pairwise agreement for isolated domain shift reason as the only difference between images within each pair is their smooth or sharp style. 
% + stat test
%}

%In all experiments, we zoom images to $1 \times 1$ mm pixel size and use additional rotations and flips augmentation. With probability $0.5$ we rotate an image by multiply of $90$ degrees and flip an image horizontally or vertically. 

%In gamma correction, we augment images using gamma transformation: 
%\[\hat{I}(x, y) = \left(\frac{I(x, y) - m}{M - m}\right)^\gamma \cdot(M - m) + m,\]
%where $M = \max(I(x, y))$, $m=\min(I(x, y))$ with a parameter $\gamma$, such that we randomly sample logarithm of $\gamma$ from $\mathcal{N}(0, 0.2)$ distrubution. 
%Gaussian noise is the additive noise from $\mathcal{N}(0, 0.1)$ distribution. 
% In random windowing we uniformly sample the center of the window $c$ from $[-700, -500]$ Hounsfield units (HU)  and the width of the window $w$ from $[1300, 1700]$ HU. Then we clip the image to the $[c - w/2, c + w/2]$ range using following formula:
% %$\mathcal{U}([-700, -500])$, $\mathcal{U}([1300, 1700])$
% \begin{equation*}
% \hat{I}(x, y) = 
%  \begin{cases}
%   c - w/2, &\text{if } I(x, y) \le c - w/2 \\
%   I(x, y, z), &\text{if } I(x, y) \in (c - w/2, c + w/2) \\
%   c + w/2, &\text{if } I(x, y) \ge c + w/2
%  \end{cases}
% \end{equation*}

% For the FBPAug we uniformly sample parameters $a$ from $[10.0, 40.0]$ and  $b$ from $[1.0, 4.0]$ in sharpening case and $a$ from $[-1.0, 0]$, $b$ from $[0.1, 1.0]$ in smoothing case. 

%Those ranges were chosen with the following procedure: first, we fix two paired images obtained using sharpening and smoothing filter; second, we use grid search with $l_2$ distance  between those images and the images transformed using FBPAug to obtain parameters resulting in best matching. 

%for arguments on these segmentation scores being on-par with the COVID-19 segmentation SOTA results, allowing for possible clinical use.

%The results of comparison with ground truth segmentation masks are presented in Tab. \ref{tab2:cancer-results-gt}. All networks were trained on the Mosmed-1110 dataset. Cross-validation results on Mosmed-1110 shows that all methods demonstrate similar segmentation quality.  As for results on the Covid-private dataset, the proposed approach outperforms the rest in terms of pairwise dice score. Recall, that in contrast  with the first column of Tab. \ref{tab2:cancer-results-gt}, the second column contains metrics measured  between paired images and not metrics with ground truth segmentation masks.





%The results of pairwise agreement comparisons are presented in Fig. \ref{fig:agreement}. .
%While we can see that in terms of Dice score three methods are no worse then the baseline, FBPAug is still outperforming others.
%FPBAug outperfoms all competitors (0.92 vs 0.54 Baseline and 0.79 gaussian noise dice scores), resulting in higher average agreement (in terms of dice score ) and lower std. \reconsider{Fig. \ref{fig:slices-contours} demonstrates that the effect is mostly due to predictions under-performs on sharper kernels (for the network trained without FBPAug)}.
%The winner become more clear when we measure the agreement  quality using Surface Dice score with different tolerancies. Even with largest tolerance ($2\text{mm}$) our method is $16\%$ better than the baseline and $9\%$ better than the closest competitor (gamma correction), with twice lower standard deviation. And for the smallest tolerance ($0.5\text{mm}$)  it is more than $26\%$ better compared to the baseline and $16\%$ better than gamma correction. Recall, that all methods, except for gaussian noise, demostrate similar or better performance compared to the baseline training without augmentation. 


==> chapters_ru/0_design_ru.tex <==
\section{Дизайн статьи}

\begin{enumerate}
    \item Введение. \textbf{(Т+А)} Описание проблемы \todo{посмотреть covid1100}, мотивация (какие то работы про ядра), Domain Shift хуе-мое. + Литобзор intensity-based аугментации + synogram based augmentation (noising/denoising).
    \item Методы. \textbf{(Т)} рассказать про FBP ровно столько сколько надо чтобы рассказать про собственный вклад. unet-backbone (берем дефолтную архитектуру и она показывает высокий результат на сегментации).
    \item Эксперименты.  (Задача сегментация легких)
    \begin{itemize}
        \item \textbf{(Т)} с аугментацией
        \item \textbf{(Т)} без аугментации
        \item \textbf{(Т)} test-time аугментации с помощью look-up table
        \item \textbf{(А)} (чуть-чуть подумать) мб. intesity-based аугментации без синограмм в исходном пространстве (если есть и легко реализовать то можно вставить, если трудно реализовать то просто упомянем в списке литературы)
    \end{itemize}
    \item Описание результатов, идеи для картинок.Таблица с результами сегментации  (разные ядра, одинаковые ядра).
    \begin{itemize}
        \item Учимся на одних ядрах тестируем на других. 
        \item Учимся на одних ядрах тестируем на тех же самых. 
        \item Учимся на всех тестируем на всех? Либо натравить Бориса, либо разметить 20-30 кейсов? \textbf{(А)}
    \end{itemize}
\end{enumerate}


\begin{enumerate}
    \item Введение
    \begin{itemize}
        \item Мотивация.
        \item Постановка задачи. Domain Adaptation, domains == convolutional kernels (CT-LDCT??).
    \end{itemize}
    \item Литобзор: тут придется еще просерчить литературу, у меня не очень много пока накопилось. Нужна литература по поводу того, что FBP действительно используется в современных томографах. Работы про разные фильтры в FBP. Поискать, пробовал ли кто-то делать что-то похожее на то, что делаем мы.
    \todo{Что такое FBP?} \textbf{FBP - Filtered Back Projection --- каноничный алгоритм для восстановления изображения по синограмме.}
    \item Методы
    \begin{itemize}
        \item Background: more or less detailed FBP algorithm description (интегральчики и матеша добавят солидности тексту, я уверен))) \todo{Это интересно, и это точно надо в журнальной версии, но я не уверен что нужно сильно расписывать в конференционной версии (но все-таки сколько-нибдуь надо, согласен)}. \textbf{Окей, ну это уже в последнюю очередь можно решить.}
        \item Наше классное преобразование в фурье спейсе. Пояснить, почему оно выглядит именно так
    \end{itemize}
    \item Постановка экспериментов
    \begin{itemize}
        \item Бейзлайн
        \item Аугментации во время обучения
        \item Возможно, использовать преобразование на построцессинге. Тут сложность в том, что надо ручками подбирать параметры преобразования, чтобы что-то получить адекватное. Я пробовал делать это для одной из версий ковидной сетки, которая работала хорошо только на определенном типе ядер. Но параметры подобрать так и не смог. Нужно попробовать это сделать на легких. \todo{А мы не можем просто сделать lookup table с каким-то количеством преобразований? И делать что-то вроде test-time augmentation (делаем все преобразования, гоним инферес, усредняем предикт)? Вероятно очень долгий инференс получится, и возможно эту часть лучше указать как future research plans (объяснив проблемой долгого инфереса).} \textbf{Хмм, да, идея мне нравится, сделаем. Посмотреть, что получится, уж точно стоит.}
    \end{itemize}
    \item Результаты
    \begin{itemize}
        \item Непосредственно само преобразование. Мб тут можно использовать какие-нибудь метрики, которые считают статистики просто по картинкам, чтобы посравнивать КТ изначально в шумном ядре с КТ в мягком ядре, которую мы превратили в шумную нашим преобразованием. Ну и картинки нарисовать, конечно. \todo{Да, думаю можно это попробовать кратко порисерчить.}
        \item Сегментация легких
    \end{itemize}
\end{enumerate}


==> chapters_ru/2_methods_ru.tex <==
 \section{Methods}
 
 In this section we give a background on a discrete version of inverse Radon Transform such as Filtered Back-Projections (FBP) algorithm. FBP consists of two sequential operations: generation of filtered projections and image reconstruction by Back-Projection operator.
 Projections of attenuation map have to be filtered before they are used as an input of Back-Projection operator. The ideal filter in continuous noiseless case is the ramp filter ($\hat{\kappa}(w) = |w|$ in Fourier domain). Although in real world manufacturers of CT scanners use different filters for reconstruction due to improving reconstruction quality by a proper filter design.
 
%  Наверное, все, что выше написанно, надо не в методы или мб переформулировать.
 
% Тут должны быть мысли по поводу того, почему формула выбрана именно такой. Это простое степенное преобразование, при этом регулируя параметры можно влиять на высокие частоты. Мягкий фильтр - приглушаем высокие частоты, резкий фильтр - наоборот, усиляем их. 
 

 Fourier transform of the proposed filter is
$$\hat{k}(w) = \hat{\kappa}(w)(1 + a \hat{\kappa}(w)^b) = |w|(1 + a|w|^b).$$
 Here $a$ and $b$ are parameters that influence sharpness or smoothness of output image. Parameter $a > 0$ corresponds enhancing high frequencies thus sharpening an image and $a < 0$ corresponds smoothing. 
 
 Алгоритм следующий. Пусть дана синограмма $s(\theta, r)$ полученная с помощью воздействия на физическое тело параллельных рентгеновских лучей под различными углами. Тогда $\theta$ - угол падения параллельных лучей, а $r$ - расстояние от луча до начала координат (начала координат в геометрическом центре тела и параметры принимают дискретный набор значений).
 Чтобы получить из синограммы изображение среза тела в декартовой системе координат, необходимо для каждого фиксированного угла применить к $s(\theta, r)$ одномерное преобразование Фурье, поточечно умножить Фурье-образ на наш предложенный фильтр.
 К полученным одномерным функциям применить обратное преобразование Фурье, получив $s(\theta, r)$. И к $s(\theta, r)$ применить back-projection algorithm. 
 %\Tilde{s}, \Tilde{s}
 To overcome filter based domain shift we propose following method. During training phase we transform an element of a batch with probability $0.25$ using our algorithm with sharpening parameters and with probability $0.25$ with smoothing parameters. В силу специфики алгоритма, преобразование может быть использовано только к целому двумерному срезу. Вследствие этого в модели присутствуют только двумерные свертки и на вход принимается батч из целых двумерных срезов изображения КТ.
 
 
 
Задача Lungs:
1.
NSCLCRadiomics -> cancer500  (4 аугментации + 1 без аугментаций) * 3 фолда, учим легкие на всем, предсказываем на парных снимках
цель: продемонстрировать что улучшается согласованность предсказаний.
по хорошему это надо пересчитать в виде:
LIDC (soft) -> cancer500 (4 аугментации + 1 без аугментаций) * 3 фолда, учим легкие на мягких, предсказываем на парных снимках
LIDC (hard) -> cancer500 (4 аугментации + 1 без аугментаций) * 3 фолда, учим легкие на жестких, предсказываем на парных снимках
Задача Cancer:
2.
LIDC (soft) -> LIDC (hard) (4 аугментации + 1 без аугментаций) * 3 фолда
LIDC (hard) -> LIDC (soft) (4 аугментации + 1 без аугментаций) * 3 фолда
цель: продемонстрировать что улучшается качество предсказаний в условиях недостатка данных с другими ядрами.
3.
LIDC (4 аугментации + 1 без аугментаций) * 3 фолда - учимся на всем, предсказываем на всем
цель: продемонстрировать что улучшается качество предсказаний даже когда нет недостатка данных с другими ядрами.
